Automatic Clone Recommendation for Refactoring Based on the Present and the Past

When many clones are detected in software programs, not all clones are equally important to developers. To help developers refactor code and improve software quality, various tools were built to recommend clone-removal refactorings based on the past and the present information, such as the cohesion degree of individual clones or the co-evolution relations of clone peers. The existence of these tools inspired us to build an approach that considers as many factors as possible to more accurately recommend clones. This paper introduces CREC, a learning-based approach that recommends clones by extracting features from the current status and past history of software projects. Given a set of software repositories, CREC first automatically extracts the clone groups historically refactored (R-clones) and those not refactored (NR-clones) to construct the training set. CREC extracts 34 features to characterize the content and evolution behaviors of individual clones, as well as the spatial, syntactical, and co-change relations of clone peers. With these features, CREC trains a classifier that recommends clones for refactoring. We designed the largest feature set thus far for clone recommendation, and performed an evaluation on six large projects. The results show that our approach suggested refactorings with 83% and 76% F-scores in the within-project and cross-project settings. CREC significantly outperforms a state-of-the-art similar approach on our data set, with the latter one achieving 70% and 50% F-scores. We also compared the effectiveness of different factors and different learning algorithms.

==> concepts.tex <==
\section{Concepts}

In this section, we define and explain the terminologies used in the paper.

When maintaining software, developers modify code and then commit those changes together with some textual description to version control systems like SVN and Git. In our paper, each code change commit is a \emph{\textbf{patch}}. The corresponding textual description is called \emph{\textbf{commit message}}.

Fig.~\ref{PatchExample} shows a patch example, which represents code changes as textual \emph{diff}s. Each textual diff describes changes applied to one file. When developers modify multiple files, the patch can contain multiple textual diffs.
\begin{figure}[!htb]
\centering
\scriptsize
\vspace{-2em}
\begin{tabular}{@{}p{0.45\textwidth}}
\begin{Verbatim}[commandchars=\\\{\}, tabsize=2]
1. diff --git a/org.eclipse.jdt.core/search/org/eclipse/jdt/
   core/search/SearchParticipant.java b/org.eclipse.jdt.core/
   search/org/eclipse/jdt/core/search/SearchParticipant.java
2. index ee39ea4..8d2f5c8 100644
3. --- a/org.eclipse.jdt.core/search/org/eclipse/jdt/core/
   search/SearchParticipant.java
4. +++ b/org.eclipse.jdt.core/search/org/eclipse/jdt/core/
   search/SearchParticipant.java
5. @@ -10,10 +10,13 @@
6.   *****************************************************/
7.   package org.eclipse.jdt.core.search;
8.
9. \color{blue}{\textbf{+ import java.io.File;}}
10.\color{blue}{\textbf{+}}
11.  import org.eclipse.core.resources.IResource;
12.  import org.eclipse.core.resources.IWorkspaceRoot;
13.  import org.eclipse.core.resources.ResourcesPlugin;
14.  import org.eclipse.core.runtime.*;
15.\color{blue}{\textbf{+ import org.eclipse.jdt.internal.core.JavaModel;}}
16.  import org.eclipse.jdt.internal.core.JavaModelManager;
17.  import org.eclipse.jdt.internal.core.search.indexing.
		IndexManager;
18.
19.@@ -173,8 +176,13 @@		
20.  public final void scheduleDocumentIndexing(SearchDocument
		document, IPath indexLocation) \{
21.    IPath documentPath = new Path(document.getPath());
22.    IWorkspaceRoot root = ResourcesPlugin.getWorkspace()
		.getRoot();
23.\color{red}{\textminus   IResource resource = root.findMember(documentPath);}
24.\color{red}{\textminus   IPath containerPath = resource == null ? documentPath :}
   \color{red}{ resource.getProject().getFullPath();}
25.\color{blue}{\textbf{+   Object file = JavaModel.getTarget(root, documentPath,}}
   \color{blue}{\textbf{ true);}}
26.\color{blue}{\textbf{+   IPath containerPath = documentPath;}}
27.\color{blue}{\textbf{+   if (file instanceof IResource) \{}}
28.\color{blue}{\textbf{+     containerPath = ((IResource)file).getProject()}}
   \color{blue}{\textbf{ .getFullPath();}}
29.\color{blue}{\textbf{+   \} else if (file == null) \{}}
30.\color{blue}{\textbf{+     containerPath = documentPath.removeLastSegments(}}
   \color{blue}{\textbf{ documentPath.segmentCount()-1);}}
31.\color{blue}{\textbf{+   \}}}
32.    IndexManager manager = JavaModelManager
		.getJavaModelManager().getIndexManager();
33.    String osIndexLocation = indexLocation.toOSString();	
34.    // TODO (jerome) should not have to create index
		manually, should expose API that recreates index instead
\end{Verbatim}
\end{tabular}
\vspace{-1em}
\caption{An exemplar patch applied to Eclipse JDT Core.}
\label{PatchExample}
\end{figure}
\vspace{-0.5em}

We defined \emph{\textbf{buggy snippet}} to describe the edit location where a bug fix was applied. Given a bug fix (or an edit fragment), the buggy snippet includes the context lines above the bug fix, the deleted lines in the fix, and the context lines below the fix. A bug fix \emph{f} is a \emph{\textbf{repeated fix}} of another one \emph{$f^{\prime}$} if \emph{f} and \emph{$f^{\prime}$} are identical or similar. A \emph{\textbf{repeated-fix group}} consists of a fix and its repeated ones.


